Compilation Semantics for a Programming Language with Versions

Programming with versions is a paradigm that allows a program to use multiple versions of a module so that the programmer can selectively use functions from both older and newer versions of a single module. Previous work formalized $\lambda_{\mathrm{VL}}$, a core calculus for programming with versions, but it has not been integrated into practical programming languages. In this paper, we propose VL, a Haskell-subset surface language for $\lambda_{\mathrm{VL}}$ along with its compilation method. We formally describe the core part of the VL compiler, which translates from the surface language to the core language by leveraging Girard's translation, soundly infers the consistent version of expressions along with their types, and generates a multi-version interface by bundling specific-version interfaces. We conduct a case study to show how VL supports practical software evolution scenarios and discuss the method's scalability.

==> figs/fig2-2.tex <==
\begin{figure}
\centering
\begin{lstlisting}[style=haskell]
-- App version 1
import Dir (exists)
import Hash (mkHash)

main () =
  let s = getArg () in
  let digest = mkHash s in
  if exists digest
    then print "Found"
    else error "Not found"
\end{lstlisting}

\begin{lstlisting}[style=haskell]
-- Dir version 1
import Hash (match)

exists hash = 
  let files = getFileList () in
  foldLeft
    (\(acc, f) ->
      acc || match f hash)
    false
    files
\end{lstlisting}

\begin{lstlisting}[style=haskell]
-- Hash version 1
mkHash s = (* generate MD5 hash *)
match s hash = (mkHash s) == hash
\end{lstlisting}

\caption{\textit{App}, \textit{Dir}, and \textit{Hash} modules \emph{before} update.}
\label{list1}
\end{figure}

==> figs/fig6-1.tex <==
\begin{figure}[t]
\begin{tikzpicture}[node distance=1.5cm, align=center
    ]
    \tikzset{%
      >={Latex[width=2mm,length=2mm]},
      % Specifications for style of nodes:
               label/.style = {fill=white, font=\sffamily},
                base/.style = {rectangle, rounded corners, draw=black,
                               minimum width=3cm, minimum height=1cm,
                               text centered, font=\sffamily},
         constraints/.style = {base, fill=green!30},
           interface/.style = {base, fill=orange!15, font=\ttfamily},
            multimod/.style = {rounded rectangle,  draw,  text centered, line width=2pt, 
                               text width=3cm, minimum height=1cm, font=\ttfamily},
           singlemod/.style = {rounded rectangle,  draw,  text centered, 
                               text width=3cm, minimum height=1cm, font=\ttfamily},
      multimodsample/.style = {rounded rectangle,  draw,  text centered, line width=2pt, 
                               text width=2cm, font=\ttfamily},
     singlemodsample/.style = {rounded rectangle,  draw,  text centered, 
                               text width=2cm, font=\ttfamily},
    }
  % Specification of nodes (position, etc.)
  \node (source) 
        [multimod]
        {VL Source};
  \node (entryAbsyn)
        [singlemod, right of=source, xshift=4cm]
        {Lang.Absyn};
  \node (entryLambdaVL)
        [singlemod, below of=entryAbsyn, yshift=-1cm]
        {Lang.LambdaVL};
  \node (duplicatedLambdaVL)
        [singlemod, below of=entryLambdaVL, yshift=-1cm]
        {Lang.LambdaVL};
  \node (inferredLambdaVL)
        [singlemod, below of=duplicatedLambdaVL, yshift=-1cm]
        {Lang.LambdaVL};
  \node (bundledLambdaVL)
        [multimod, below of=inferredLambdaVL, yshift=-1cm]
        {Lang.LambdaVL};
  \node (specifiedLambdaVL)
        [multimod, below of=bundledLambdaVL, yshift=-1cm] 
        {Lang.LambdaVL};
  \node (endAbsyn)
        [multimod, below of=specifiedLambdaVL, yshift=-1cm] 
        {Lang.Absyn};
  \node (typeinfo)
        [interface, right of=inferredLambdaVL, xshift=2.5cm]
        {Syntax.Type};
  \node (interface)
        [interface, below of=typeinfo, yshift=-1cm]
        {Syntax.Env\\(Interface)};
  \node (Constraints)
        [constraints, left of=duplicatedLambdaVL, xshift=-4cm]
        {Constraints};
  \node (Vectors)
        [constraints, below of=Constraints, yshift=-1cm]
        {Vectors};
  \node (labels)
        [singlemod, left of=bundledLambdaVL, xshift=-4cm]  
        {Labels};
  \node (HsSyn)
        [multimod, left of=endAbsyn, xshift=-4cm]
        {GHC.HsSyn};  

  \node (sampleSingle) 
        [singlemodsample, right of=entryAbsyn, xshift=3cm]
        {Single module};
  \node (sampleMulti) 
        [multimodsample, right of=entryAbsyn, xshift=3cm, yshift=-1.2cm]
        {Multiple modules};

  % Specification of lines between nodes specified above
  % with aditional nodes for description 
  \draw[->]             (source) -- node[font=\sffamily,midway,below]
                                    {parser\\and\\dependency\\analyser} (entryAbsyn);
  \draw[->]         (entryAbsyn) -- node[label]{girardFwd}
                                    (entryLambdaVL);
  \draw[->]      (entryLambdaVL) -- node[label](duplication)
                                    {Duplication} (duplicatedLambdaVL);
  \draw[->] (duplicatedLambdaVL) -- node[label](typeinference)
                                    {Type Inference} (inferredLambdaVL);
  \draw[->]   (inferredLambdaVL) -- node[label](bundling)
                                    {Bundling} (bundledLambdaVL);
  \draw[->]      (typeinference) -| (typeinfo);
  \draw[->]           (typeinfo) -- node[label] {Bundling} (interface);
  \draw[->]      (typeinference) -- ++ (-2.5, 0) |- (Constraints);
  \draw[->]           (bundling) -- ++ (-2.5, 0) |- (Constraints);
  \draw[->]        (Constraints) -- node[label] {Vectorize} (Vectors);
  \draw[->]            (Vectors) -- node[label] {z3} (labels);
  \draw[->]    (bundledLambdaVL) -- (specifiedLambdaVL);
  \draw[->]  (specifiedLambdaVL) -- node[label] {girardBck} (endAbsyn);
  \draw[->]          (interface) -- ++ (2,0) |- node[label] {import} (duplication);
  \draw[->]        (labels) -- ++ (0,-1) -| node [font=\sffamily, below, pos=0.25]
                                                      {Version\\specialization}
                                                 (specifiedLambdaVL);
  \draw[->]           (endAbsyn) -- (HsSyn);
  % \draw[->]    (bundledLambdaVL) -| node(priorityXMemory)
  %                                   {higher priority $\rightarrow$ more memory}
  %                                   (Constraints);
  % \draw[->]      (Constraints)  |- node [yshift=-2cm, text width=3.1cm]
  %                                   {User navigates back to the activity}
  %                                   (absyn);
  % \draw[->] (bundledLambdaVL.east) -- ++(2.6,0) -- ++(0,2) -- ++(0,2) --                
  %    node[xshift=1.2cm,yshift=-1.5cm, text width=2.5cm]
  %    {The activity comes to the foreground}(duplicatedLambdaVL.east);
  \end{tikzpicture}
  \caption{The pipeline of VL Language System}
  \label{fig:pipeline}
\end{figure}

==> rules/rule_constraints_generation.tex <==
\begin{figure*}[tb]
  \centering
  \hrule
  \medskip
  \begin{tabular}{l}
    \begin{minipage}{.9\linewidth{}}
        \textbf{\vlmini{} constraints generation \ \ \ 
        \fbox{\ensuremath{\Sigma \,\vdash\, \alpha \sqsubseteq_{c} [\Gamma] \rhd \mathcal{C}}}}
    \end{minipage}
    \medskip\\
    \begin{minipage}{.35\linewidth}
      \infrule[$\emptyset$]{
        % \Sigma \,\vdash\, \alpha : \textsf{Labels}
        \\
      }{
        \Sigma \,\vdash\, \alpha \sqsubseteq_{c} \emptyset \rhd \top
      }
    \end{minipage}
    \begin{minipage}{.60\linewidth}
      \infrule[$\alpha$]{
        % \Sigma \,\vdash\, \alpha : \textsf{Labels}
        % \andalso
        \Sigma \,\vdash\, \alpha \sqsubseteq_{c} [\Gamma] \rhd \mathcal{C}
      }{
        \Sigma \,\vdash\, \alpha \sqsubseteq_{c} (x:[A]_r , [\Gamma]) \rhd (\alpha \preceq r \land \mathcal{C})
      }
    \end{minipage}
  \end{tabular}
  \medskip
  \hrule

  \caption{\vlmini{} constraints generation}
  %\ecaption{Typing of \corelang}
  % \Description{\corelang algorithmic typing}
  \label{fig:rule_constraints_generation}
\end{figure*}

==> rules/rule_context_grading.tex <==
\begin{figure*}[t]
    \centering
    \hrule
    \vspace{.3em}
    \begin{tabular}{lccc}
        \begin{minipage}{.9\linewidth{}}
            \textbf{\vlmini{} context grading \ \ \ 
            \fbox{\ensuremath{\Sigma \,\vdash\, [\Gamma]_{\textsf{Labels}} \rhd \Gamma'}}}
        \end{minipage}
        \\\\
        \begin{minipage}{.40\linewidth}
            \infrule[$\emptyset$]{
                \\
            }{
                \Sigma \,\vdash\, [\emptyset]_{\textsf{Labels}} \rhd \emptyset
            }
        \end{minipage}
        % \\\\
        \begin{minipage}{.55\linewidth}
            \infrule[{[}lin{]}]{
                \Sigma \,\vdash\, [\Gamma]_{\textsf{Labels}} \rhd \Gamma'
            }{
                \Sigma \,\vdash\, [\Gamma,x:A]_{\textsf{Labels}} \rhd \Gamma', x:[A]_\emptyset
            }
        \end{minipage}
        \\\\
        \begin{minipage}{.95\linewidth}
            \infrule[{[}gr{]}]{
                \Sigma \,\vdash\, [\Gamma]_{\textsf{Labels}} \rhd \Gamma'
            }{
                \Sigma \,\vdash\, [\Gamma,x:[A]_r]_{\textsf{Labels}} \rhd \Gamma', x:[A]_{r}
            }
        \end{minipage}
    \end{tabular}
    \vspace{.5em}
    \hrule
    \medskip
    \caption{\vlmini{} context grading}
    %\ecaption{Typing of \corelang}
    % \Description{\corelang algorithmic typing}
\label{fig:rule_context_grading}
\end{figure*}

==> rules/rule_data_structure.tex <==
\begin{figure*}[t]
  \centering
  \hrule
  \medskip
  \begin{tabular}{c}
    \begin{minipage}{.9\linewidth{}}
        \textbf{\vlmini{} algorithmic type inference \ \ \ \fbox{\ensuremath{\Sigma;\Gamma \vdash t \Rightarrow A;\Sigma';\theta; \mathcal{C}}}}
    \end{minipage}
    \\\\
    \begin{minipage}{.95\linewidth}
      \infrule[$\Rightarrow_{\textsc{(,)}}$]{
        \Sigma_{i-1};\Gamma \vdash t_i \Rightarrow A_i; \Sigma_i; \theta_i; \mathcal{C}_i
      }{
        \Sigma_0;\Gamma \,\vdash\, (t_1,\,..\,,t_n) \Rightarrow (A_1,\,..\,,A_n); \Sigma_{n};\biguplus_{i=1}^n\theta_{i}; \bigwedge_{i=1}^n \mathcal{C}_i
      }
    \end{minipage}
    \\\\
    \begin{minipage}{.95\linewidth}
      \infrule[$\Rightarrow_{\textsc{[,]}}$]{
        \Sigma_{i-1};\Gamma \vdash t_i \Rightarrow A; \Sigma_i; \theta_i; \mathcal{C}_i
      }{
        \Sigma_0;\Gamma \,\vdash\, [t_1,\,..\,,t_n] \Rightarrow [A]; \Sigma_{n};\biguplus_{i=1}^n\theta_{i}; \bigwedge_{i=1}^n \mathcal{C}_i
      }
    \end{minipage}
    \\\\
    \begin{minipage}{.95\linewidth}
      \infrule[$\Rightarrow_{\textsc{case}}$]{
        \Sigma_{0};\Gamma \vdash t \Rightarrow A; \Sigma_1; \theta_0; C_0
        \andalso\\
        \Sigma_{i-1};- \vdash p_{i}:A \rhd \Delta_{i}; \Sigma'_{i}; \theta'_{i}
        \andalso
        \Sigma'_{i};\Gamma,\Delta_{i} \vdash t_{i} \Rightarrow B;\Sigma_{i};\theta_{i}; \mathcal{C}_{i}
      }{
        \Sigma_0;\Gamma \,\vdash\, \caseof{t}{\overline{p_i\mapsto t_i}} \Rightarrow (\biguplus_{i=0}^n\theta_{i})B;\Sigma_{n};\biguplus_{i=0}^n\theta_{i}; \bigwedge_{i=0}^n \mathcal{C}_i
      }
    \end{minipage}
    \\\\
    \begin{minipage}{.9\linewidth{}}
        \textbf{\vlmini{} pattern type synthesis \ \ \ 
        \fbox{\ensuremath{\Sigma, R\,\vdash\, p : A \rhd \Gamma; \Sigma'; \theta}}}
    \end{minipage}
    \\\\
    \begin{minipage}{.95\linewidth}
      \infrule[pCon]{
        \Sigma_{i-1}' = \Sigma_{i-1}, \alpha_i:\textsf{Type}
        \andalso
        \Sigma_{i-1}'; - \vdash p_i : \alpha_i \rhd \Gamma_i; \Sigma_i; \theta_i
        \andalso\\
        \Sigma_n \vdash K\,\alpha_1,\,..\,\alpha_n \sim A \rhd \theta'
      }{
        \Sigma_0; - \,\vdash\, C\,p_1\,..\,p_n : A \rhd \Gamma_i, .. ,\Gamma_n; \Sigma_n; \theta'\uplus\biguplus_{i=1}^n\theta_{i}
      }
    \end{minipage}
    \\\\
    \begin{minipage}{.95\linewidth}
      \infrule[\mbox{[}pCon\mbox{]}]{
        \Sigma_{i-1}' = \Sigma_{i-1}, \alpha_i:\textsf{Type}
        \andalso
        \Sigma_{i-1}'; r \vdash p_i : \alpha_i \rhd \Gamma_i; \Sigma_i; \theta_i
        \andalso\\
        \Sigma_n \vdash K\,\alpha_1,\,..\,\alpha_n \sim A \rhd \theta'
        \andalso
        \Sigma_i' \,\vdash\, r : \textsf{Labels}
      }{
        \Sigma_0; r \,\vdash\, C\,p_1\,..\,p_n : A \rhd \Gamma_i, .. ,\Gamma_n; \Sigma_n; \theta'\uplus\biguplus_{i=1}^n\theta_{i}
      }
    \end{minipage}
    \\\\
    \begin{minipage}{.9\linewidth{}}
        \textbf{\vlmini{} type unification \ \ \ 
        \fbox{\ensuremath{\Sigma \vdash A \sim B \rhd \theta }}}
    \end{minipage}
    \\\\
    \begin{minipage}{.95\linewidth}
      \infrule[$U_{Con}$]{
        \Sigma \,\vdash\, A_1 \sim B_1 \rhd \theta_1
        \andalso
        \Sigma \,\vdash\, \theta_{i-1} A_i \sim \theta_{i-1} B_i \rhd \theta_i
      }{
        \Sigma \,\vdash\, K\,A_1\,..\,A_n \sim K\,B_1\,..\,B_n \rhd \biguplus_{i=1}^n\theta_{i}}
    \end{minipage}
  \end{tabular}
  \medskip
  \hrule
  \caption{Extension for algorithmic typing inference, pattern type synthesis, and type unification for data strutcures.}
  %\ecaption{Typing of \corelang}
  % \Description{\corelang algorithmic typing}
  \label{fig:rule_data_stcture}
\end{figure*}

==> rules/rule_pattern_synthesis.tex <==
\begin{figure*}[t]
  \centering
  \hrule
  \smallskip
  \begin{tabular}{c}
    \begin{minipage}{.9\linewidth{}}
        \textbf{\vlmini{} pattern type inference (excerpt) \ \ \ 
        \fbox{\ensuremath{\Sigma, R\,\vdash\, p : A \rhd \Gamma; \Sigma'; \theta}}}
    \end{minipage}
    \smallskip\\
    % \begin{minipage}{.55\linewidth}
    %   \infrule[\mbox{[}p\_\mbox{]}]{
    %     \Sigma \,\vdash\, r : \textsf{Labels}
    %     \andalso
    %     \Sigma \,\vdash\, A : \textsf{Type}\\
    %   }{
    %     \Sigma; r \,\vdash\, \_ : A \rhd \emptyset; \Sigma; \emptyset
    %   }
    % \end{minipage}
    % \\\\
    % \begin{minipage}{.45\linewidth}
    %   \infrule[pInt]{
    %     \\
    %   }{
    %     \Sigma; - \,\vdash\, n : \inttype \rhd \emptyset; \Sigma; \emptyset
    %   }
    % \end{minipage}
    % \begin{minipage}{.50\linewidth}
    %   \infrule[\mbox{[}pInt\mbox{]}]{
    %     \Sigma \,\vdash\, r : \textsf{Labels}
    %   }{
    %     \Sigma; r \,\vdash\, n : \inttype \rhd \emptyset; \Sigma; \emptyset
    %   }
    % \end{minipage}
    % \\\\
    \begin{minipage}{.45\linewidth}
      \infrule[pVar]{
        \Sigma \,\vdash\, A : \textsf{Type}
      }{
        \Sigma; - \,\vdash\, x : A \rhd x:A; \Sigma; \emptyset
      }
    \end{minipage}
    \begin{minipage}{.50\linewidth}
      \infrule[\mbox{[}pVar\mbox{]}]{
        \Sigma \,\vdash\, A : \textsf{Type}
        \andalso
        \Sigma \,\vdash\, r : \textsf{Labels}
      }{
        \Sigma; r \,\vdash\, x : A \rhd x:\verctype{A}{r}; \Sigma; \emptyset
      }
    \end{minipage}
    \\\\
    \begin{minipage}{.95\linewidth}
      \infrule[p$\square$]{
        \Sigma' = \Sigma, \alpha:_\exists\textsf{Labels}, \beta:_\exists\textsf{Type}
        \andalso
        \Sigma' \,\vdash\, \alpha : \textsf{Labels}
        \andalso\\
        \Sigma'; \alpha \,\vdash\, p : \beta \rhd \Delta; \Sigma''; \theta
        \andalso
        \Sigma' \,\vdash\, A \sim \vertype{\alpha}{\beta} \rhd \theta'
      }{
        \Sigma; - \,\vdash\, [p] : A \rhd \Delta; \Sigma''; \theta \uplus \theta'
      }
    \end{minipage}
    \\\\
    \begin{minipage}{.95\linewidth}
      \infrule[\mbox{[}p$\square$\mbox{]}]{
        \Sigma' = \Sigma, \alpha:_\exists\textsf{Labels}, \beta:_\exists\textsf{Type}
        \andalso
        \Sigma' \,\vdash\, \alpha : \textsf{Labels}
        \andalso\\
        \Sigma'; r \otimes \alpha \,\vdash\, p : \beta \rhd \Delta; \Sigma''; \theta
        \andalso
        \Sigma' \,\vdash\, A \sim \vertype{\alpha}{\beta} \rhd \theta'
        % \textsf{flatten}(r,R,r',R')=(s,S)
      }{
        \Sigma; r \,\vdash\, [p] : A \rhd \Delta; \Sigma''; \theta\uplus\theta'
      }
    \end{minipage}
  \end{tabular}
  \smallskip
  \hrule

  \caption{\vlmini{} pattern type synthesis}
  %\ecaption{Typing of \corelang}
  % \Description{\corelang algorithmic typing}
  \label{fig:rule_pattern_synthesis}
\end{figure*}

==> rules/rule_semantics.tex <==
\begin{figure*}[t]
    \centering
    \hrule
    \medskip
    \begin{tabular}{c}
        \begin{minipage}{.9\linewidth{}}\textbf{Evaluation rule}\end{minipage}
        \\\\
        \begin{minipage}{.95\linewidth}
            \infrule[]{
                t \leadsto t'
            }{
                E[t] \longrightarrow E[t']
            }
        \end{minipage}
    \end{tabular}
    \medskip
    \hrule
    \medskip
    \begin{tabular}{c}
        \begin{minipage}{.9\linewidth{}}\textbf{Reduction rules}\end{minipage}
        \\\\
        \begin{minipage}{.35\linewidth}
            \infrule[E-abs]{
                \\
            }{
                \app{(\lam{x}{t})}{t'} \leadsto (t' \rhd x)t
            }
        \end{minipage}
        \begin{minipage}{.50\linewidth}
            \infrule[E-clet]{
                \\
            }{
                \clet{x}{v}{t} \leadsto (v \rhd \pr{x})t
            }
        \end{minipage}
        \\\\
        \begin{minipage}{.25\linewidth}
            \infrule[E-ex1]{
                \\
            }{
                \pr{t}.l \leadsto t@l
            }
        \end{minipage}
        \begin{minipage}{.35\linewidth}
            \infrule[E-ex2]{
                \\
            }{
                \{\overline{l=t}\,|\,l_k\}.l_i \leadsto t_i@l_i
            }
        \end{minipage}
        \begin{minipage}{.35\linewidth}
            \infrule[E-veri]{
                \\
            }{
                \langle\overline{l=t}\,|\,l_k\rangle \leadsto t_k@l_k
            }
        \end{minipage}
    \end{tabular}
    \medskip
    \hrule
    \medskip
    \begin{tabular}{c}
        \begin{minipage}{.9\linewidth{}}\textbf{Substitutions}\end{minipage}
        \\\\
        \begin{minipage}{.32\linewidth}
            \infrule[\ensuremath{\rhd_{\mathrm{var}}}]{
                \\
            }{
                (t' \rhd x) t = [t'/x]t
            }
        \end{minipage}
        \begin{minipage}{.30\linewidth}
            \infrule[\ensuremath{\rhd_{\square}}]{
                %(t \rhd p)t = t'
                (t \rhd x)t' = t''
            }{
                %([t] \rhd [p])t = t'
                ([t] \rhd [x])t' = t''
            }
        \end{minipage}
        \\\\
        \begin{minipage}{.55\linewidth}
            \infrule[\ensuremath{\rhd_{\mathrm{ver}}}]{
                \\
            }{
                (\{\overline{l=t}\,|\,l_i\} \rhd [x]) t = [\langle\overline{l=t}\,|\,l_i\rangle/x] t
            }
        \end{minipage}
    \end{tabular}
    \medskip
    \hrule
    \medskip
    \begin{tabular}{c}
        \begin{minipage}{.9\linewidth{}}\textbf{Default version overwriting}\end{minipage}
        \\\\
        \begin{minipage}{.12\linewidth}
            \infax[]{
                n@l \,\equiv\, n
            }
        \end{minipage}
        \begin{minipage}{.12\linewidth}
            \infax[]{
                x@l \,\equiv\, x
            }
        \end{minipage}
        \begin{minipage}{.28\linewidth}
            \infax[]{
                (\lam{x}{t})@l \,\equiv\, \lam{x}{(t@l)}
            }
        \end{minipage}
        \begin{minipage}{.28\linewidth}
            \infax[]{
                (\app{t}{u})@l \,\equiv\, \app{(t@l)}{(u@l)}
            }
        \end{minipage}
        \\\\
        \begin{minipage}{.60\linewidth}
            \infax[]{
                \clet{x}{t_1}{t_2}@l \,\equiv\, \clet{x}{(t_1@l)}{(t_2@l)}
            }
        \end{minipage}
        \\\\
        \begin{minipage}{.18\linewidth}
            \infax[]{
                \pr{t}@l \,\equiv\, \pr{t}
            }
        \end{minipage}
        \begin{minipage}{.40\linewidth}
            \infax[]{
                \{\overline{l=t}\,|\,l_i\}@l' \,\equiv\, \{\overline{l=t}\,|\,l_i\}
            }
        \end{minipage}
        \begin{minipage}{.25\linewidth}
            \infax[]{
                (t.l)@l' \,\equiv\, (t@l').l
            }
        \end{minipage}
        \\\\
        \begin{minipage}{.40\linewidth}
            \infrule[]{
                l' \in \{\overline{l}\}
            }{
                \langle\overline{l=t}\,|\,l_i\rangle@l' \,\equiv\, \langle\overline{l=t}\,|\,l'\rangle
            }
        \end{minipage}
        \begin{minipage}{.40\linewidth}
            \infrule[]{
                l' \notin \{\overline{l}\}
            }{
                \langle\overline{l=t}\,|\,l_i\rangle@l' \,\equiv\, \langle\overline{l=t}\,|\,l_i\rangle
            }
        \end{minipage}
    \end{tabular}
    \medskip
    \hrule
    \caption{\corelang dynamic semantics}
    %\ecaption{Typing rules of \corelang}
    \label{fig:rule_semantics}
\end{figure*}

\begin{comment}
\begin{tabular}{c}
    \begin{minipage}{.60\linewidth}
        \infrule[\ensuremath{\rhd_{\square}}]{
            (v \rhd p)t = t'
        }{
            ([v] \rhd [p])t = t'
        }
    \end{minipage}
\end{tabular}
\end{comment}
\begin{comment}
\begin{tabular}{c}
    \begin{minipage}{.9\linewidth}
        \infrule[\ensuremath{\rhd_C}]{
            (v_i \rhd p_i)t_i = t_{i+1}
        }{
            (C\ v_0..v_n \rhd C\ p_0..p_n)t_0 = t_{n+1}
        }
    \end{minipage}
\end{tabular}
\end{comment}
\begin{comment}
    &
    \begin{minipage}{.21\linewidth}
        \infrule[app$_R$]{
            t_2 \leadsto t_2'
        }{
            t_1\ t_2 \leadsto t_1\ t_2'
        }
    \end{minipage}
\end{comment}
\begin{comment}
    &
    \begin{minipage}{.21\linewidth}
        \infrule[$\square$]{
            t \leadsto t'
        }{
            [t] \leadsto [t']
        }
    \end{minipage}
\end{comment}

==> rules/rule_subsumption.tex <==
\begin{figure*}[t]
\centering
\hrule
\smallskip
\begin{tabular}{c}
    \begin{minipage}{.9\linewidth{}}\textbf{Subsumption rules}\end{minipage}
    \\\\
    \begin{minipage}{.30\linewidth}
        \infrule[]{
            \\
        }{
            A \,<:\, A
        }
    \end{minipage}
    \begin{minipage}{.30\linewidth}
        \infrule[]{
            A \,<:\, B
            \andalso
            r' \,\sqsubseteq\, r
        }{
            \vertype{r}{A} \,<:\, \vertype{r'}{B}
        }
    \end{minipage}
    \begin{minipage}{.35\linewidth}
        \infrule[]{
            A' \,<:\, A
            \andalso
            B \,<:\, B'
        }{
            \ftype{A}{B} \,<:\, \ftype{A'}{B'}
        }
    \end{minipage}
    \\\\
    \begin{minipage}{.35\linewidth}
        \infrule[]{
            A \,<:\, B
            \andalso
            r' \,\sqsubseteq\, r
        }{
            \verctype{A}{r} \,<:\, \verctype{B}{r'}
        }
    \end{minipage}
    \begin{minipage}{.20\linewidth}
        \infrule[]{
            \\
        }{
            \Gamma \,\sqsubseteq\, \Gamma
        }
    \end{minipage}
    \begin{minipage}{.35\linewidth}
        \infrule[]{
            \Gamma \,\sqsubseteq\, \Delta
            \andalso
            A \,<:\, B
        }{
            \Gamma, x:B \,\sqsubseteq\, \Delta, x:A
        }
    \end{minipage}
\end{tabular}
\medskip
\hrule
\caption{Subsumption rules for typing context}
%\ecaption{Typing rules of \corelang}
\label{fig:rule_subsumption}
\end{figure*}

==> rules/rule_typing.tex <==
\begin{figure*}[t]
\centering
\hrule
\medskip
\begin{tabular}{c}
    \begin{minipage}{.9\linewidth{}}\textbf{\corelang{} typing rules \ \ \ \fbox{\ensuremath{\Gamma \,\vdash\, t:A}}}\end{minipage}
    \\\\
    \begin{minipage}{.30\linewidth}
        \infrule[int]{
             \\% \\
        }{
            \emptyset \,\vdash\, n : \textsf{Int}
        }
    \end{minipage}
    \begin{minipage}{.30\linewidth}
        \infrule[var]{
            \\
        }{
            x:A \,\vdash\, x:A
        }
    \end{minipage}
    \begin{minipage}{.35\linewidth}
        \infrule[abs]{
            \Gamma, x:A \,\vdash\, t : B%\theta B
        }{
            \Gamma \,\vdash\, \lam{x}{t} : \ftype{A}{B}
        }
    \end{minipage}
    \\\\
    \begin{minipage}{.95\linewidth}
        \infrule[app]{
            \Gamma_1 \,\vdash\, t_1 : \ftype{A}{B}
            \andalso
            \Gamma_2 \,\vdash\, t_2 : A
        }{
            \Gamma_1 + \Gamma_2 \,\vdash\, \app{t_1}{t_2} : B
        }
    \end{minipage}
    \\\\
    \begin{minipage}{.95\linewidth}
        \infrule[let]{
            \Gamma_1 \,\vdash\, t_1 : \vertype{r}{A}
            \andalso
            \Gamma_2, x:\verctype{A}{r} \,\vdash\, t_2 : B
        }{
            \Gamma_1 + \Gamma_2 \,\vdash\, \clet{x}{t_1}{t_2} : B
        }
    \end{minipage}
    \\\\
    \begin{minipage}{.30\linewidth}
        \infrule[weak]{
            \Gamma \,\vdash\, t : A
        }{
            \Gamma, \verctype{\Delta}{0} \,\vdash\, t : A
        }
    \end{minipage}
    \begin{minipage}{.35\linewidth}
        \infrule[der]{
            \Gamma, x:A \,\vdash\, t : B
        }{
            \Gamma, x:\verctype{A}{1} \,\vdash\, t : B
        }
    \end{minipage}
    \begin{minipage}{.30\linewidth}
        \infrule[pr]{
            [\Gamma] \,\vdash\, t : A 
        }{
            r\cdot[\Gamma] \,\vdash\, [t] : \vertype{r}{A} 
        }
    \end{minipage}
    \\\\
    \begin{minipage}{.50\linewidth}
        \infrule[sub]{
            \Gamma,x:\verctype{A}{r}, \Gamma' \,\vdash\, t : B
            \andalso
            r \sqsubseteq s
        }{
            \Gamma,x:\verctype{A}{s}, \Gamma' \,\vdash\, t : B
        }
    \end{minipage}
    \begin{minipage}{.45\linewidth}
        \infrule[extr]{
            \Gamma \,\vdash\, t : \vertype{r}{A}
            \andalso
            l \in r
        }{
            \Gamma \,\vdash\, t.l : A
        }
    \end{minipage}
    \\\\
    \begin{minipage}{.95\linewidth}
        \infrule[ver]{
            [\Gamma_i] \,\vdash\, t_i : A
        }{
            \bigcup_i(\{l_i\}\cdot [\Gamma_i]) \,\vdash\, \{\overline{l=t}\,|\,l_i\} : \vertype{\{\overline{l}\}}{A}
        }
    \end{minipage}
    \\\\
    \begin{minipage}{.95\linewidth}
        \infrule[veri]{
            [\Gamma_i] \,\vdash\, t_i : A
        }{
            \bigcup_i(\{l_i\}\cdot [\Gamma_i]) \,\vdash\, \langle\overline{l=t}\,|\,l_i\rangle : A
        }
    \end{minipage}
\end{tabular}
\medskip
\hrule
\caption{\corelang typing rules}
%\ecaption{Typing rules of \corelang}
\label{fig:rule_typing}
\end{figure*}

==> rules/rule_unification.tex <==
\begin{figure*}[t]
  \centering
  \hrule
  \medskip

  \begin{tabular}{c}
    \begin{minipage}{.9\linewidth{}}
        \textbf{\vlmini{} type unification \ \ \ 
        \fbox{\ensuremath{\Sigma \vdash A \sim B \rhd \theta }}}
    \end{minipage}
    \\\\
    \begin{minipage}{.95\linewidth}
      \infrule[$U_\rightarrow$]{
        \Sigma \,\vdash\, A' \sim A \rhd \theta_1
        \andalso
        \Sigma \,\vdash\, \theta_1B\sim \theta_1B' \rhd \theta_2
      }{
        \Sigma \,\vdash\, A \rightarrow B \sim A' \rightarrow B' \rhd \theta_1 \uplus \theta_2
      }
    \end{minipage}
    \\\\
    %  &
    % \begin{minipage}{.20\linewidth}
    %   \infrule[$U_{\textsc{Con}}$]{
    %     \\
    %   }{
    %     \Sigma \,\vdash\, K \sim K \rhd \emptyset
    %   }
    % \end{minipage}
    \begin{minipage}{.95\linewidth}
      \infrule[$U_{\Box}$]{
        \Sigma \,\vdash\, A \sim A' \rhd \theta_1
        \andalso
        \Sigma \,\vdash\, \theta_1 r \sim \theta_1 r' \rhd \theta_2
      }{
        \Sigma \,\vdash\, \vertype{r}{A} \sim \vertype{r'}{A'} \rhd \theta_1\uplus\theta_2}
    \end{minipage}
    \\\\
    \begin{minipage}{.95\linewidth}
      \infrule[$U_{\textsc{Var}\exists}$]{
        (\alpha:\kappa) \in \Sigma
        \andalso
        \Sigma \vdash A:\kappa
      }{
        \Sigma \,\vdash\, \alpha \sim A \rhd \alpha \mapsto A
      }
    \end{minipage}
    \\\\
    \begin{minipage}{.47\linewidth}
      \infrule[$U_{\textsc{Var}=}$]{
        (\alpha:\kappa) \in \Sigma\\
      }{
        \Sigma \,\vdash\, \alpha \sim \alpha \rhd \emptyset
      }
    \end{minipage}
    \begin{minipage}{.48\linewidth}
      \infrule[$U_{=}$]{
        \Sigma \vdash A:\kappa
      }{
        \Sigma \,\vdash\, A \sim A \rhd \emptyset      }
    \end{minipage}
  \end{tabular}
  \medskip
  \hrule
  \medskip

  \caption{\vlmini{} type unification}
  %\ecaption{Typing of \corelang}
  % \Description{\corelang algorithmic typing}
  \label{fig:rule_unification}
\end{figure*}

==> syntax/versioninference.tex <==
\begin{figure}[tb]
\begin{align*}
\Gamma & ::= \emptyset \,\mid\, \Gamma, x:A \,\mid\, \Gamma, x:\verctype{A}{r} \tag{typing contexts}\\
\Sigma & ::= \emptyset \,\mid\, \Sigma, \alpha:\kappa \tag{type variable kinds}\\
R      & ::= - \,\mid\, r \tag{resource contexts}
\end{align*}
\caption{The syntax of \vlmini{} for algorithmic version inference.}
\label{syntax:versioninference}
\end{figure}
